Software for cut-generating functions in the Gomory--Johnson model and beyond

We present software for investigations with cut generating functions in the Gomory-Johnson model and extensions, implemented in the computer algebra system SageMath.

==> Makefile <==
LATEX=latex
PDFLATEX=pdflatex
FIG2DEV=fig2dev
BIBTEX=bibtex

FIGURESDIRPREFIX=

MAINTEXFILE=software-abstract

all: $(MAINTEXFILE).pdf

%.pstex_t: %.fig #Makefile
	$(FIG2DEV) -L pstex_t -p $*.pstex $< $@

%.pstex: %.fig #Makefile
	$(FIG2DEV) -L pstex $< $@

%.pdftex_t: %.fig #Makefile
	$(FIG2DEV) -L pdftex_t -p $*.pdf $< $@

%.pdf: %.fig #Makefile
	$(FIG2DEV) -L pdftex $< $@

SOFTWARE_ABSTRACT_GRAPHICS_SOURCES=

SOFTWARE_ABSTRACT_GENERATED_GRAPHICS=$(SOFTWARE_ABSTRACT_GRAPHICS_SOURCES:%.fig=$(FIGURESDIRPREFIX)%.pdftex_t) $(SOFTWARE_ABSTRACT_GRAPHICS_SOURCES:%.fig=$(FIGURESDIRPREFIX)%.pdf) 

#$(SOFTWARE_ABSTRACT_GRAPHICS_SOURCES:%.fig=%.pstex_t) $(SOFTWARE_ABSTRACT_GRAPHICS_SOURCES:%.fig=%.pstex)

SOFTWARE_ABSTRACT_SOURCES=Makefile $(MAINTEXFILE).tex $(SOFTWARE_ABSTRACT_GRAPHICS_SOURCES:%.fig=$(FIGURESDIRPREFIX)%.fig) \
	sage-commands.tex

SOFTWARE_ABSTRACT_STYLES = llncs.cls

## copied these files from their source:
## $ (cd ~/Dropbox/yuan-group-relaxation-sage-code/ && tar cf - $files) | tar xvf -
SOFTWARE_ABSTRACT_GRAPHICS=$(SOFTWARE_ABSTRACT_GENERATED_GRAPHICS)						\
	graphics-for-algo-paper/2d_diagram_with_cones_continuous_deco.png					\
	graphics-for-algo-paper/2d_diagram_with_cones_discontinuous.png						\
	graphics-for-algo-paper/2d_with_cones_discontinuous.png							\
	graphics-for-algo-paper/2d_with_faces_discontinuous.png							\
	graphics-for-algo-paper/construct_a_face.png

# copy-graphics-from-dropbox:
# 	(cd $$HOME/Dropbox/yuan-group-relaxation-sage-code/ && tar cf - $(SOFTWARE_ABSTRACT_GRAPHICS)) | tar xvf -

BIB=../../bib/MLFCB_bib.bib

.PHONY: figures

figures: $(SOFTWARE_ABSTRACT_GRAPHICS) 

$(MAINTEXFILE).pdf: $(MAINTEXFILE).tex $(SOFTWARE_ABSTRACT_GRAPHICS) $(BIB)
	$(PDFLATEX) -halt-on-error "$<"
	$(BIBTEX) $(MAINTEXFILE)
	$(PDFLATEX) -halt-on-error "$<"
	$(PDFLATEX) -halt-on-error "$<"

SOFTWARE_ABSTRACT_SOURCES_AND_MORE=$(SOFTWARE_ABSTRACT_SOURCES) $(SOFTWARE_ABSTRACT_GRAPHICS) $(SOFTWARE_ABSTRACT_STYLES)

.PHONY: arxiv
arxiv:
	COPYFILE_DISABLE=true tar -cf $(CURDIR)/$(MAINTEXFILE).tar	\
		$(MAINTEXFILE).bbl					\
		$(SOFTWARE_ABSTRACT_SOURCES)					\
		$(SOFTWARE_ABSTRACT_GRAPHICS)					\
		$(SOFTWARE_ABSTRACT_STYLES)
	rm -f $(MAINTEXFILE).tar.gz
	gzip $(MAINTEXFILE).tar

